QPTAS for Geometric Set-Cover Problems via Optimal Separators

Weighted geometric set-cover problems arise naturally in several geometric and non-geometric settings (e.g. the breakthrough of Bansal-Pruhs (FOCS 2010) reduces a wide class of machine scheduling problems to weighted geometric set-cover). More than two decades of research has succeeded in settling the $(1+\epsilon)$-approximability status for most geometric set-cover problems, except for four basic scenarios which are still lacking. One is that of weighted disks in the plane for which, after a series of papers, Varadarajan (STOC 2010) presented a clever \emph{quasi-sampling} technique, which together with improvements by Chan \etal~(SODA 2012), yielded a $O(1)$-approximation algorithm. Even for the unweighted case, a PTAS for a fundamental class of objects called pseudodisks (which includes disks, unit-height rectangles, translates of convex sets etc.) is currently unknown. Another fundamental case is weighted halfspaces in $\Re^3$, for which a PTAS is currently lacking. In this paper, we present a QPTAS for all of these remaining problems. Our results are based on the separator framework of Adamaszek-Wiese (FOCS 2013, SODA 2014), who recently obtained a QPTAS for weighted independent set of polygonal regions. This rules out the possibility that these problems are APX-hard, assuming $\textbf{NP} \nsubseteq \textbf{DTIME}(2^{polylog(n)})$. Together with the recent work of Chan-Grant (CGTA 2014), this settles the APX-hardness status for all natural geometric set-cover problems.

==> applications.tex <==
 %%%%% \begin{theorem}
%%%%% \label{thm:setcover}
%%%%% Let $\mathcal{R}$ be a set of $n$ weighted $\alpha$-simple regions let $P$ be a finite set of points in the plane. There exists a $(1+\epsilon)$-approximation for computing the minimum weight subset of $\mathcal{R}$ that covers $P$, that runs in time $(\alpha n)^{O(\alpha\phi(n)\log^2{(n/\epsilon)}/\epsilon)}$.
%%%%% \end{theorem}



\section{QPTAS for Independent Set. Proof of Theorem~\ref{thm:indepset}}
\label{sec:mis}


We start with the problem of computing the maximum independent of regions in the plane. This was already done by Adamaszek and Weise for a class of regions in the plane~\cite{AW13,AW14}. We extend their results to a more general class of regions and improve the running time of their algorithm.  We then extend their technique to get a QPTAS for other problems. In these application, the main technical tool is a suitable separator. The rest of the algorithmic ideas are similar to that of  Adamaszek and Weise except that we don't use dynamic programming. Our description of the algorithm will therefore be brief and we only describe it for the first application. For the rest of the applications, we only show the existence of a separator and the algorithm remains the same. 

Let $\mathcal{R}$ be a set of $n$ weighted regions in  plane, each region $R\in \mathcal{R}$. Let $\textsc{Opt}(\mathcal{R})$ denote a subset $\mathcal{Q} \subseteq \mathcal{R}$ pairwise disjoint regions maximizing the total weight $w(\mathcal{Q})$. Given any parameter $0<\epsilon < 1$, our goal is to compute a set $\mathcal{Q}' \subseteq \mathcal{R}$ of pairwise disjoint regions such that  $w(\mathcal{Q}') \geq (1-\epsilon) w(\textsc{Opt}(\mathcal{R}))$. 

For ease of exposition, we first explain the algorithm for a simple class of regions i.e., when $\mathcal{R}$ is a set of line segments in the plane. The ideas easily generalize to a set of $\alpha$-simple regions where $\alpha = \polylog (n)$.

 By a suitable choice of axes, we can ensure that no line segment is vertical, i.e., each segment is $1$-simple. If the maximum weight of the segments is $M$, then $w(\textsc{Opt}(\mathcal{R}))$ is at least $M$, and the segments of weight $\epsilon M/n$ together contribute a weight of at most $\epsilon M$. Thus, we can ignore the segments of weight less than $\epsilon M/n$ and assume that the minimum weight of any segment is at least $\epsilon M/n$. By scaling the weights, we may assume that the minimum weight of the segments is $1$ and the maximum weight is at most $n/\epsilon$ and thus $w(\textsc{Opt}(\mathcal{R})) \leq n^2/\epsilon$. 

 Consider the set $\mathcal{Q}=\textsc{Opt}(\mathcal{R})$. If we apply Theorem~\ref{thm:weightedseparator} to the set $\mathcal{Q}$ for parameter $\delta = \epsilon$, we get a separator $\C$ so that that the weight of segments in $\mathcal{Q}$ intersecting $\C$ is at most $\delta w(\mathcal{Q})$.
  Furthermore, $w(\mathcal{Q}_{in})$ and $w(\mathcal{Q}_{ext})$ are at most $\frac{2}{3} w(\mathcal{Q})$.
   Assuming $\delta \leq \frac{1}{6}$, by the optimality of $\mathcal{Q}$, $w(\textsc{Opt}(\mathcal{R}_{in})) \leq w(\mathcal{Q}_{in}) + w(\mathcal{Q}_{bd}) \leq \frac{5}{6} w(\textsc{Opt}(\mathcal{R}))$. Similarly  $w(\textsc{Opt}(\mathcal{R}_{ext})) \leq \frac{5}{6} w(\textsc{Opt}(\mathcal{R}))$. Also note that $\textsc{Opt}(\mathcal{R}_{in}) \cup \textsc{Opt}(\mathcal{R}_{ext})$ gives a valid solution to the problem and has weight at least $(1-\epsilon) w(\textsc{Opt}(\mathcal{R}))$. 
  
    Thus, if we could   guess the separator $\C$, we could use it for divide and conquer.
   We can ignore the segments in $\mathcal{R}$ that intersect $\C$ and recursively compute approximate solutions for the set of segments in $interior(\C)$ and $exterior(\C)$.
  If the recursive solutions are exact, then the weight of the solution returned is at least  $(1-\epsilon)w(\mathcal{Q})$.
  However, the recursive solutions are not exact and there is a loss incurred at every level of recursion. 
 Since the weight of the optimal solution falls by a constant factor with every recursion, we only need $O(\log{n^2/\epsilon}) = O (\log{n/\epsilon})$ levels in the recursion tree. 
 To compensate for the loss at every level of recursion, we set $\delta = \Theta(\epsilon/\log{(n/\epsilon)})$. Since we do not have a way to compute the separator $\C$, at any level of recursion, we try all possible separators. By Theorem~\ref{thm:weightedseparator}, the separator can be encoded by a sequence of $O(1/\delta)$ elements of $\mathcal{R}$ and $O(1/\delta)$ additional bits. Thus there are at most $t=O(n^{O(1/\delta)})$ candidate separators to try. 
 The algorithm is thus as follows. Starting with the given set of segments $\mathcal{R}$, we enumerate and try all of the (at most $t$) separators each of which gives us two recursive problems. We prune the recursion tree at the level $l = O (\log{n/\epsilon})$ since we know that for the  right  choice of separators at each recursion, these many levels are sufficient. The size of the tree is at most $(2t)^l = O(n^{\log^2{(n/\epsilon)}/\epsilon})$. Our recursion tree contains, as a subtree, the tree that corresponds to choosing the right separator at every recursion. Call the nodes of this tree ``good nodes''. We now work bottom up in our recursion tree. 
 
At the bottom level, for the subproblems that correspond to good nodes, the weight of the maximum independent set is at most $1$. Since the weight of any segment is at least $1$, this means that the size of the maximum independent set is at most $1$ and thus can be found in polynomial time. At every bottom level subproblem, we return the segment of the maximum weight if the subproblem is non-empty. We return an empty set otherwise. This certainly gives the right answer for the good nodes. For the other nodes, the answer may not be optimal but it is certainly a valid independent set.

 Once we have solved the sub-problems corresponding to a node in the recursion tree, we take ``best'' solution among the solutions provided by the different choice of separators. Note that the best solution to a good node may come from nodes that are not good nodes. The solution is still a valid solution and at least as good as that coming from good nodes.
The good nodes thus always get a solution of the desired approximation. It can be shown inductively that the approximation factor at a good node that is $k$ levels away from the lowest level is $(1-\delta)^k$. Thus the approximation factor at the root is $(1-\delta)^l \geq (1-\epsilon)$ since we have chosen $\delta = c\epsilon/l$ for a suitably large constant $c$. The time taken by the algorithm is $O(n^{\log^2{(n/\epsilon)}/\epsilon})$. Since this analysis of the running time and approximation factor has been done in \cite{AW13} and \cite{AW14}, we do not elaborate on this further. 

Two technical details have been swept under the rug in the description above. The first is that for the existence of the separator for the set $\mathcal{Q}$, we require that all elements of $\mathcal{Q}$ have weight at most $w(\mathcal{Q})/3$. It may not always be the case. Assume that there exists some $Q \in \mathcal{Q}$ with weight more than $w(\mathcal{Q})/3$. However, since we are producing all possible separators, we will also produce a separator $\C$ whose interior contains just $Q$ and whose boundary does not intersect any segment from $\mathcal{Q}$. The subproblem corresponding to $exterior(\C)$ is still fine since the weight of the segments in it drops by a constant factor.
The subproblem in $interior(\C)$ has an optimal solution of size $1$ and therefore 
a simple modification to the algorithm takes care of such subproblems. After we compute the ``best'' solution to a node in the recursion tree, we compare it with the segment of the maximum weight in the subproblem. We return the better of the two.
 
 The second problem is that segments from $interior(\C)$ and $exterior(\C)$ may touch at $\C$ since we don't consider a segment whose end point is on $\C$ as intersecting $\C$. Thus the two subproblems are not really independent, i.e., we cannot compute independent sets in each separately and take the union. This problem is easily solved by first streching each input segment $s$ slightly to $s'$ such that $s$ lies in the relative interior of $s'$ and the intersection graph of the segments does not change, and then applying the algorithm to the stretched segments.

Since Theorem~\ref{thm:weightedseparator} works for arbitrary $\alpha$-simple regions in the plane, everything described above generalizes for $\alpha$-simple regions in the plane.
The number of curves is now $O(\alpha n)$ since each of the $n$ regions is $\alpha$ simple.
 We also gain a factor of $\alpha$ in the encoding size of the separator and hence also in the exponent in the running time. Thus we obtain Theorem~\ref{thm:indepset}.


\section{QPTAS for Geometric Set Cover Problems. Proof of Theorem~\ref{thm:setcover}.}
\label{sec:gsc}

Let $\R = \{R_1, \ldots, R_n\}$ be a set of $n$ weighted regions in the plane and let $P$ be a finite set of points in the plane. The goal is to compute a subset $\mathcal{Q} \subseteq \mathcal{R}$ minimizing the total weight $w(\mathcal{Q})$ so that $P\subseteq \cup_{Q\in \mathcal{Q}}Q$. We will denote the weight of
an optimal solution $\mathcal{Q}$ for an instance of the problem given by a set of regions $\mathcal{R}$ and a set of points $P$ by $\textsc{Opt}(\mathcal{R}, P)$.

% {\bf Cite papes of Kasturi, Chan et al - PTAS not known for weighted set cover of disks}. 

We show that for pseudodisks in the plane, there exists a QPTAS for the problem. 
To do so, we show the existence of a suitable separator using Theorem~\ref{thm:weightedseparator} and then use the divide and conquer strategy as described in the previous section. 

\begin{claim}
\label{claim:tofame}
%Let $(\R, P)$ be the given set-system, where $R \in \R$ has weight $w(R)$.
%Then 
If there exists a QPTAS for set-systems $(\R', P')$ 
where each $R \in \R'$ has weight $w(R) \geq 1$, and the weight
of the optimal set-cover for $(\R', P')$ is $O(n/\eps)$, 
then there exists a QPTAS for the minimum-weight set cover
for a set-system $(\R, P)$ with arbitrary weights.
%and $w(\sum_{R \in \R'} w(R) \leq n/\epsilon$
%
%Then one can construct a new set system $(\R', P')$ in
%polynomial time, where each $R \in \R'$ has weight $w(R) \geq 1$,
%and $\sum_{R \in \R'} w(R) \leq n/\epsilon$ such that,
%from a set-cover $\Q'$ to $(\R', P')$, one can construct
%a set-cover for $(\R, P)$ in polynomial time of total weight $(1 + \eps) w_{opt}(\R)$.
\end{claim}
\begin{proof}
Let $\Q$ be a minimum-weight set-cover for $(\R, P)$. First guess the maximum weight region
in $\Q$, say of weight $w_{max}$ (there are $n$ such choices). Then by exponential search on the 
interval $[w_{max}, nw_{max}]$, one can guess the weight of $\Q$ within a $(1+\eps/3)$ factor (there are $O(\log_{1+\eps}n)$ such
choices). Let $w_{apx}$ be this weight, satisfying
$w(\Q) \leq w_{apx} \leq (1+\eps/3)w(\Q)$.
Set $\R' \subset \R$ to be the set of regions with
weight at least $\eps w_{apx}/n$, and $\R'' = \R \setminus \R'$.
Let $P' \subseteq P$ be the set of points not covered by $\R''$,
and construct a $(1+\eps/3)$ approximate set-cover $\Q'$
to $(\R', P')$. Return $\Q' \cup \R''$ as a set-cover
for $(\R, P)$. Note that this is the required approximation:
\begin{eqnarray*}
w(\Q' \cup \R'') = w(\Q') + w(\R'') &\leq& (1+\eps/3)w(\Q_{opt}(\R', P')) + \eps w_{apx} \\
& \leq &(1+\eps/3) w(\Q) + \eps (1+\eps/3) w(\Q) \leq (1+\eps)w(\Q)
\end{eqnarray*}
Above we use the fact that $\Q$ is also a set-cover for $(\R', P')$. This further
implies that, by scaling, each set in $\R'$ has weight at least $1$, 
and the scaled weight of $w(\Q)$ is $O(n/\eps)$.


%Scaling up the weights in $\R'$ by $1/(\eps w_{approx}/n)$ makes
%the minimum weight in $\R'$ at least one, and the 
%
%Add each region of $\R$ with weight in the range $[\epsilon w_{approx}/2n, w_{max}]$ to $\R'$. 
%Scaling up gives us the required $\R'$.
%Let $P'$ be the set of points not covered by regions of weight at most $\epsilon w_{max}/n$
%in $\R$.
%%These regions in $\R'$ have weight in the range
%%$[\eps w_{max}/n, nw_{max}]$. 
%Returning a (1+\eps/2)-approximate set-cover $\Q'$ for $(\R', P')$ together the sets
%in $\R$ of weight at most $\epsilon w_{max}/2n$
% yields the required set cover for $\R$ of total weight $w(\Q') + \eps w_{max} = w(\Q') + \eps w_{opt}(\R)
% \leq (1+\eps)w_{opt}(\R)$.
\end{proof}

Hence for the purpose of a $(1+\epsilon)$-approximation, we can assume that the minimum weight of any region is $1$ and the  weight of the optimal set-cover
is at most $O(n/\epsilon)$. 
%
%This is because all the regions of weight at most an $\epsilon/n$-fraction of the maximum weight can be added to the solution without affecting the weight of the solution by more than a factor of $(1+\epsilon)$ .  Thus the weight of the optimal solution is at most $n^2/\epsilon$.


\input{setcover.tex}





%%%
%%%\begin{theorem}
%%%Let $\mathcal{R}$ be a set of $\alpha$-simple regions in the plane with union complexity $\phi(\cdot)$ such that none of the regions lies in the union of the others. Let $w(R)$ be a positive weight assigned to each region $R \in \mathcal{R}$ so that no region is assigned a weight more than a third of the total weight $W=\sum_{R \in \mathcal{R}}w(R)$. Then, for any parameter $0 < \beta < \frac{1}{6}$, there exists a closed curve $\C$ and a constant $A$ such that 
%%%\begin{itemize}
%%%\item $\C$ can be completely described by sequence of $O(\alpha \phi(n)/\beta)$ curves in $\Gamma(\mathcal{R})$ and $O(\alpha \phi(n)/\beta)$ extra bits,
%%%\item the total weight of the regions in $\mathcal{R}$ whose cores intersect $\C$ is at most $\beta \ W$.
%%%\item the total weight of the regions in $\mathcal{R}$ whose cores lie in $interior(\C)$ is at most $(1 - \frac{1}{A\alpha\phi(n)})W$,
%%%\item the total weight of the regions in $\mathcal{R}$ whose cores lie in $exterior(\C)$ is at most $(1 - \frac{1}{A\alpha\phi(n)})W$, and
%%%\end{itemize}
%%%\end{theorem}
%%%
%%%\begin{proof}
%%%For each $R \in \mathcal{R}$, let $\Gamma(\tilde{R})$ be the set given by Theorem~\ref{thm:cores}. Let $\mathcal{D} = \bigcup_{R\in \mathcal{R}} \Gamma(\tilde{R})$.
%%%Note that interiors of any pair of curves in $D$ are disjoint.
%%%For each $D \in \mathcal{D}$, there are at most two regions $R$ such that $D \in \Gamma(\tilde{R})$. Assign to $D$ a weight $w(D)$ equal to the sum of the weights of these regions. 
%%%The boundary of each core consists of at most $O(\alpha \phi(n)) = C\alpha\phi(n)$ curves in $\mathcal{D}$, for some constant $C$. Therefore, the total weight of all curves in $\mathcal{D}$ is $W' \leq C\alpha \phi(n) W$. Also, since   no region in $\mathcal{R}$ lies in the union of the other regions, no core is empty and therefore, the boundary of each core has at least two curves. This implies that $W' \geq 2W$. Since no region in $\mathcal{R}$ has weight more than $W/3$, no $D \in \mathcal{D}$ has weight more than $2W/3 \leq W'/3$. Applying Theorem~\ref{thm:separator} to the curves in$\mathcal{D}$, with the weights we have defined and  $\delta = \frac{\beta}{C\alpha \phi(n)}$, we get the required curve $\C$. $\C$ is completely described by $O(1/\delta)$ curves in $\mathcal{D}$ and $O(\frac{1}{\delta})$ extra bits. Since each curve in $\mathcal{D}$ is described by at most three curves in $\Gamma(\mathcal{R})$ and a constant number of bits, the first item in the statement of the theorem follows.
%%% 
%%%The total weight of the curves in $\mathcal{D}$ that intersect $\mathcal{C}$ is at most $\delta W' = \beta W$. Therefore the total weight of the regions whose cores intersect $\C$ is also at most $\beta W$. That proves the second item in the statement of the theorem follows.
%%%
%%% Let $\mathcal{R}_{in} \subseteq \mathcal{R}$ denote the set of regions 
%%% whose cores lie in $interior(\C)$. Let $W(\mathcal{R}_{in}) = \sum_{R \in \mathcal{R}_{in}} w(R)$. Similarly let $\mathcal{D}_{in} \subseteq \mathcal{D}$ denote set of curves in $\mathcal{D}$ that lie in $interior(C)$ and let $W(\mathcal{D}_{in}) = \sum_{D \in \mathcal{D}_{in}} w(D)$. Since the boundary of the core of every region in $\mathcal{R}_{in}$ consists of at most $C\alpha\phi(n)$ curves in $\mathcal{D}$, $W(\mathcal{R}_{in}) \geq \frac{W(\mathcal{D}_{in})}{C\alpha\phi(n)}$. Theorem~\ref{thm:separator} guarantees that $ W(\mathcal{D}_{in}) \geq (\frac{1}{3} - \delta) W' \geq \frac{W'}{6}$ since $\delta \leq \beta \leq \frac{1}{6}$. Thus $W(\mathcal{R}_{in}) \geq \frac{W'}{6C\alpha\phi(n)} \geq \frac{W}{3C\alpha\phi(n)}$. Setting $A=3C$, we conclude the third item in the statement of the theorem. The fourth item is proved analogously. 
%%%\end{proof}

\section{QPTAS for Maximum $k$-packings. Proof of Theorem~\ref{thm:kpacking}.}

Consider the following generalization of the independent set problem: Given a set $\mathcal{R}$ of $n$ (unweighted) regions and a constant parameter $k$, compute the subset $\mathcal{Q}\subseteq \mathcal{R}$ of the maximum cardinality so that no point in the plane is contained in more than $k$ regions in $\mathcal{Q}$. 
For this problem, we obtain an approximation scheme for $\alpha$-simple regions with subquadratic union complexity $n \phi(n)$.

 Consider any optimal solution $\mathcal{Q}$ for the problem. Since every vertex in the arrangement of $\mathcal{Q}$ has depth at most $k$, the number of intersections is at most $m=O(nk \phi(n))$ by the standard Clarkson-Shor technique.  We will get a suitable separator for this problem using Theorem~\ref{thm:separator}. As before, we will guarantee that there exists a separator that splits the problem in such a way that the size of the optimal solution in each subproblem goes down by a constant factor, so that the depth of the recursion tree is $O(\log{n}/\epsilon)$. We set $\delta=\epsilon/\log{(n/\epsilon)}$. Assuming $n$ is much larger than $k$ and $1/\epsilon$, we have $k \leq c_1 \delta^2 n/\phi(n)$ for any constant $c_1$ so that $m\leq c_1\delta^2n^2$. 
 
  To invoke Theorem~\ref{thm:separator}, we set $r = c_2 \alpha^2/\delta^2$ for some constant $c_2$. With a suitable constants, $c_1$ and $c_2$, we get a separator $\C$ that intersects at most $\delta$ fraction of regions in $\mathcal{Q}$, and the size of the optimal solution drops by a constant factor in both subproblems induced by $\C$. The separator $\C$ is described by a sequence of $O(\alpha/\delta)$ curves in $\cup_{R\in\mathcal{R}}\Gamma(R)$ and $O(\alpha/\delta)$ additional bits. Therefore the number of separators to try at every subproblem is $(\alpha n)^{O(\alpha/\delta)}$. By an algorithm similar to that in Section~\ref{sec:mis}, we have Theorem~\ref{thm:kpacking}. 
  
  {\bf Remark:} The only use we made of the low union complexity is in showing that the number of intersections in the optimal solutions is small. This allows us to use Theorem~\ref{thm:separator}. This method can thus be used in any situation where the optimal solution has a small number of intersections. 

==> setcover.tex <==
%\section{Set-cover}


%\subsection{Unweighted pseudodisks}




\begin{figure}
\centering
\begin{minipage}{.33\textwidth}
  \centering
  \includegraphics[width=7cm]{twodisks.pdf}
  \captionof{figure}{Pseudodisks $X$ and $Y$}
  \label{fig:twodisks}
\end{minipage}%
\begin{minipage}{.33\textwidth}
  \centering
  \includegraphics[width=7cm]{twodisks1.pdf}
  \captionof{figure}{$X$ and $Y\setminus X$ }
  \label{fig:twodisks1}
\end{minipage}
\begin{minipage}{.33\textwidth}
	\centering
	\includegraphics[width=7cm]{twodisks2.pdf} 
	\captionof{figure}{$X$ and $\tilde{Y}$}
	\label{fig:twodisks2} 
\end{minipage}
\end{figure}



\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=9cm]{threedisks.pdf}
  \captionof{figure}{Pseudodisks $X$, $Y$ and $Z$}
  \label{fig:threedisks}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=9cm]{threedisks1.pdf}
  \captionof{figure}{$\tilde{X}, \tilde{Y}$ and $\tilde{Z}$}
  \label{fig:threedisks1}
\end{minipage}
\end{figure}

The key to the application of separators for set-cover
will be the notion of \emph{core decompositions}. 
Informally, our goal is to shrink these pseudodisks in such a way that their union remains unchanged but the number of vertices in the arrangement
decreases. Suppose that we are given two pseudodisks as in Figure~\ref{fig:twodisks} and we want to remove both the intersections while retaining the union. We could keep $X$ as it is and replace $Y$ by $\tilde{Y} = closure(Y \setminus X)$ as shown in Figure~\ref{fig:twodisks1}. This keeps the union unchanged but $X$ and $\tilde{Y}$ now share a portion of their boundaries and thus technically do not form pseudodisks. To circumvent this problem, we replace our requirement that the union be unchanged with the requirement that any point that does not lie too close to the boundary of any of the pseudodisks is still covered. Then we can construct $\tilde{Y}$ as shown in Figure~\ref{fig:twodisks2}. Motivated by this, we have the definitions below. We denote by $B_\tau$ a closed ball of radius $\tau$. 
We denote the Minkowski sum by $\oplus$.


\begin{defn}
Given $\R = \{R_1, \ldots, R_n\}$ and a $\beta>0$, a set of regions $\tilde{\R} = \{\tilde{R}_1, \ldots, \tilde{R}_n\}$
is called a \emph{$\beta$-core decomposition} of $\R$ (and each
$\tilde{R}_i$ a \emph{core} of $R_i$) if
\begin{enumerate}
\item $\tilde{R}_i \subseteq R_i$ for all $i=1, \ldots, n$.
\item $\bigcup_i \tilde{R}_i \supseteq \bigcup_i {R}_i \setminus \bigcup (\partial R \oplus B_\beta) \}$
\item $\{\tilde{R}_1, \ldots, \tilde{R}_n\}$ are pseudodisks.
\end{enumerate}
\end{defn}

The following two Lemmas show the existence of core decompositions
with specific properties. 

\begin{lemma}
\label{lemma:pusher}
Given a set $\R$ of pseudodisks, 
and a marked pseudodisks $X \in \R$ (called
the \emph{pusher}), there exists a 
core decomposition $\tilde{\R}$ of $\R$ such 
that $\tilde{X} = X$ and $\tilde{R}\cap \tilde{X} = \emptyset$
for all $R \neq X$.
\end{lemma}
\begin{proof}
Informally, the pseudodisk $X$ pushes the other pseudodisks out of its region just as the pseudodisk $X$ pushes the pseudodisk $Y$ out of its region in Figure~\ref{fig:twodisks2}. We now want to show that $X$ can push all the pseudodisks out in such a way that the entire collection still forms a set of pseudodisks.
In the case of two pseudodisks we can set $\tilde{Y}$ to be $closure(Y \setminus (X \oplus B_\mu))$ where $\mu$ is some small enough number less than $\beta$ chosen so that $\tilde{Y}$ remains a pseudodisk. In this case we say that $X$ pushes $Y$ with gap $\mu$. Now, suppose that we have three pseudodisks as shown in Figure~\ref{fig:threedisks}. We now want to push $Y$ and $Z$ out of $X$. However, if we push with the same gap $\mu$ then $\tilde{Y}$ and $\tilde{Z}$ would share a portion of their boundaries. We therefore need to push different gaps $\mu_Y$ and $\mu_Z$ to ensure that $\tilde{Y}$ and $\tilde{Z}$ are pseudodisks. In this case it does not matter whether $\mu_Y$ is smaller or $\mu_Z$ is smaller. However if the pseudodisks were as shown in Figure~\ref{fig:threedisks2}, then we must pick $\mu_Y$ to be smaller than $\mu_Z$ otherwise $\tilde{Y}$ and $\tilde{Z}$ would be piercing each other and hence not form a set of pseudodisks. Now we formally describe the way to push when there are an arbitrary number of pseudodisks.

Set $\tilde{X} = X$.
For any $R \in \R$, let $I_R$ be the interval $R \cap \partial X$ on the boundary of $X$.
As no pseudodisk in $\R$ is completely contained in any other
pseudodisk of $\R$, the intervals $I_R$ are well-defined. 

Consider the partial order $\preceq$ on these intervals
defined by inclusion. We say that $I_R \preceq I_S$ if $I_R \subset I_S$ By a topological sorting of this partial order we can assign a distinct rank $rank(R) \in \{1,\cdots,n\}$ to each pseudodisk $R \in \R$ such that if $I_R \subset I_{R'}$ then $rank(R) > rank(R')$. 
We will show that it suffices to push each pseudodisk $R \in \R$ with gap $gap(R) = \mu \frac{rank(R)}{n}$ where $0< \mu < \beta$ is suitably small. In other words, for any $R \in \R$, we can set $\tilde{R} = closure (R \setminus  ( X \oplus B_{gap(R)}))$.

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=9cm]{threedisks2.pdf}
  \captionof{figure}{Pseudodisks $X$, $Y$ and $Z$}
  \label{fig:threedisks2}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=9cm]{threedisks3.pdf}
  \captionof{figure}{$\tilde{X}, \tilde{Y}$ and $\tilde{Z}$}
  \label{fig:threedisks3}
\end{minipage}
\end{figure}

%%%
%%%and let $Chain(R)$
%%%be length of the longest chain starting at $I_R$ in this partial order
%%%(i.e., $Chain(R) =i$ iff there are exactly $i$ other nested intervals containing $I_R$). Set $\tilde{R} = R \setminus \{ X \oplus B(\lambda \cdot Chain(R)) \}$,
%%%where $B(r)$ is a ball of radius $r$, and $\lambda$ is an arbitrarily
%%%small constant.
%%%See Figure~\ref{fig:coredecomposition} for an illustration.
%%%
%%%\begin{figure}[tb]
%%%\begin{center}
%%%\includegraphics[height=5cm]{coredecomposition.pdf} 
%%%\end{center}
%%%\label{fig:coredecomposition} 
%%%\end{figure}

Clearly each core is contained in its corresponding pseudodisk. Also, since the points we may have removed from the union, due to the gaps, lie in $X \oplus B_\mu$, the second condition in the definition of  a $\beta$-core decomposition is satisfied.It remains to show that the cores form pseudodisks. Let $Y$ and $Z$ be any two pseudodisks in $\R$, and we now finish
the proof by showing
that the boundaries of $\tilde{Y}$ and $\tilde{Z}$ intersect at most twice. The possible cases are the following:
\begin{enumerate}
\item $I_Y \cap I_Z = \emptyset$.
\item $I_Y \preceq I_Z$.
\item $I_Y \cap I_Z \neq \emptyset$ and $I_Y \npreceq I_Z$.
\end{enumerate}

In case $1$, since the intervals are disjoint, $\partial \tilde{Y}$ and $\partial \tilde{Z}$ do not have any new intersection that $\partial Y$ and $\partial Z$ did not have. They may have lost intersections lying in $X$. In any case, $\partial \tilde{Y}$ and $\partial \tilde{Z}$ intersect at most twice. In case $2$, $Y$ gets pushed with a smaller gap than $Z$ and the situation is exactly as shown in Figures ~\ref{fig:threedisks2} and ~\ref{fig:threedisks3}. In case $3$, $Y$ and $Z$ get pushed with different gaps and the situation is exactly as shown in Figures ~\ref{fig:threedisks} and ~\ref{fig:threedisks1}.
\end{proof}
\textbf{Remark:} Note that for each pseudodisk $R$ intersecting $X$ and not contained in $X$, 
the boundary of $\tilde{R}$ now has two new vertices corresponding to the two intersections
of $R$ with $X$. These vertices are slightly perturbed from the intersections because of 
the gap.

In the following, we will use the term {\em core decomposition} to mean a $\beta$-core decomposition with a suitably small $\beta > 0$.


\begin{lemma}
\label{lemma:coredecomposition}
Given a set of pseudodisks $\R = \{R_1, \ldots, R_n\}$
and a parameter $\eta > 0$, there exists
a core decomposition of $\R$, say the set $\tilde{\R} = \{\tilde{R}_1,
\ldots, \tilde{R}_n\}$, such that 
\begin{enumerate}
%\item the maximum depth of the arrangement induced by $\tilde{\R}$ is $O(\delta^2 n / \log^2 n)$, and
\item the number of intersections in the arrangement
induced by $\tilde{\R}$ is $O(1/\eta^2 + \eta n^2)$, and
\item the number of vertices of each pseudodisk in $\tilde{\R}$ is $O(1/\eta^2)$.
\end{enumerate}
\end{lemma}
\begin{proof}
Construct an $\eta$-net, say the set $Q = \{Q_0, \ldots,
Q_t\}$, for $\R$. By
the result of Clarkson-Varadarajan~\cite{CV05}, $Q$ 
has size $O(1/\eta)$.

Let $\R_0 = \R$. Apply Lemma~\ref{lemma:pusher} (with $Q_0 \in \R_0$ as the pusher) 
to get a core decomposition, denoted by $\R_1$,
of $\R_0$. Now apply Lemma~\ref{lemma:pusher} on $\R_1$
(with $\tilde{Q}_1 \in \R_1$ as the pusher) to get the set
$\R_2$. 
Continuing iteratively by applying
Lemma~\ref{lemma:pusher} with the successive core of each $Q_i$ in
$\R_i$ as the pusher,
we get the set $\R_t$. Replace all 
the cores of pseudodisks $R \in Q$ in $\R_t$ by $R$ to get the set $\tilde{\R}$.

Observe that each $\tilde{R} \in \tilde{\R}$ 
is disjoint from each object in $Q$ (it became
disjoint from $Q_i$ latest at the $i$-th iteration). 
As $Q$ was an $\eta$-net, any point
in the plane not covered by the union of $Q$ has
depth at most $\eta n$.
Recall that by the Clarkson-Shor technique, as pseudodisks have linear union complexity,
the maximum number of vertices at depth at most $k$ is $O(nk)$.
Therefore the total number of intersections in $\tilde{\R}$
is 
$$O(|Q|^2 + |\R_t| \cdot \eta n) = O(1/\eta^2 + n \cdot \eta n)$$

This proves condition $1$.

For condition $2.$, from the proof of Lemma~\ref{lemma:pusher},
each boundary vertex of any core object corresponds to a vertex of the arrangement
induced by the objects in $Q$. As every pair of pseudodisks
can intersect at most twice, there are $O(1/\eta^2)$ vertices
in the arrangement of $Q$.
\end{proof}

Before we prove our next main result on core decompositions,
we will need the following technical result. 
Given $\R$, the \emph{depth} of a vertex $(v,i,j)$, denoted $d_v$,
is the total weight of the regions in $\R$ containing $(v,i,j)$ in the interior
(thus it excludes the weight of $R_i$ and $R_j$).

\begin{claim}
\label{claim:cs}
Let $\R = \{R_1, \ldots, R_n\}$ be a set of $n$ weighted pseudodisks,
and $k>0$ a given parameter. 
Assume $R_i$ has weight $w_i$, and $W = \sum_i w_i$. Further let 
$(v,i,j)$ denote a vertex $v$ in the arrangement of $\R$ defined by $R_i$
and $R_j$. Then
$$ \sum_{\substack{(v,i,j) \text{ s.t. } \\ k \leq d_v < 2k}} 
\frac{w_i \cdot w_j}{w_i+w_j+k} = O(W) $$
\end{claim}
\begin{proof}
Let $\R_1 \subset \R$ be the set of disks with weight $w_i \geq 2k$, and $\R_2 = \R \setminus \R_1$.
Note that $|\R_1| = O(W/k)$, and that any vertex $v$ with depth less than $2k$
and defined by two disks in $\R_1$ must lie on the union boundary of $\R_1$. This implies 
$$ \sum_{\substack{(v,i,j) \text{ s.t. } R_i,R_j \in \R_1 \\ k \leq d_v < 2k}} 
\frac{w_i \cdot w_j}{w_i+w_j+k} \leq \sum_{\substack{(v,i,j) \text{ s.t. } R_i,R_j \in \R_1 \\ k \leq d_v < 2k}} 
\min \{w_i, w_j \} =  O(\sum_{R_i \in \R_1} w_i) = O(W)$$
where the second-last inequality follows from the fact that
the number of vertices in the union for $t$ pseudodisks is $O(t)$, 
and so each vertex can be assigned to one of its two disks such that
each disk gets $O(1)$ assigned vertices. 

The proof for the remaining vertices
follows from a standard application of the Clarkson-Shor technique.
Set $S = \R_1$, and add each disk $R_i \in \R_2$ into $S$
with probability $p_i = w_i/4k$. Then
$$ \text{Expected union complexity of S} = E[ O( |S| ) ] = O(|\R_1| + \sum_{R_i \in \R_2} \frac{w_i}{4k}) = O(W/k)$$
On the other hand, the expected number of vertices
defined by the intersection
of a disk in $\R_2$ and a disk in $\R_1$, and of depth less than $2k$,
that end up as vertices in the union of $S$:
\begin{eqnarray*}
\sum_{\substack{(v,i,j) \text{ s.t. } R_i \in \R_2, R_j \in \R_1 
\\ k \leq d_v < 2k}} \frac{w_i}{4k} \prod_{\substack{R_l \text{ contains } v
\\ R_l \in \R_2}}
(1-p_l) 
\geq \sum \frac{w_i}{4k} e^{-2\sum_l w_l/4k}  
\geq 
\sum \frac{w_i}{4ek}
\end{eqnarray*}
using the fact that $1-x \geq e^{-2x}$ for $0 \leq x \leq 0.5$,
and that $\sum w_l \leq 2k$ as all such $R_l$ contain $v$, which has
depth at most $2k$.
The expected number of vertices in the union of $S$ 
defined by two disks in $\R_2$, and of depth at most $2k$:
\begin{eqnarray*}
\sum_{\substack{(v,i,j) \text{ s.t. } R_i \in \R_2, R_j \in \R_2 
\\ k \leq d_v < 2k}} \frac{w_i}{4k} \cdot \frac{w_j}{4k} \prod_{\substack{R_l \text{ contains } v \\ R_l \in \R_2}} (1-p_l) 
\geq \sum \frac{w_i \cdot w_j}{16ek^2}
\end{eqnarray*}
Putting the lower- and upper-bounds together, we arrive at:
$$ 
\sum_{\substack{(v,i,j) \text{ s.t. } R_i \in \R_2, R_j \in \R_1}} \frac{w_i}{4ek} +
\sum_{\substack{(v,i,j) \text{ s.t. } R_i \in \R_2, R_j \in \R_2}} \frac{w_i \cdot w_j}{16ek^2} 
\leq O(W/k)$$

Finally, 
\begin{eqnarray*}
\sum_{\substack{(v,i,j) \text{ s.t. } \\ k \leq d_v < 2k}} 
\frac{w_i \cdot w_j}{w_i+w_j+k} &=& 
\sum_{\substack{(v,i,j) \\ R_i \in \R_2, R_j \in \R_1}}
 \frac{w_i \cdot w_j}{w_i+w_j+k} + \sum_{\substack{(v,i,j) \\ R_i \in \R_2, R_j \in \R_2}}
 \frac{w_i \cdot w_j}{w_i+w_j+k}  \\ 
 && + \sum_{\substack{(v,i,j) \\ R_i \in \R_1, R_j \in \R_1}}
 \frac{w_i \cdot w_j}{w_i+w_j+k} \\
 & \leq & 
 \sum_{\substack{(v,i,j) \\ R_i \in \R_2, R_j \in \R_1}}
 w_i + \sum_{\substack{(v,i,j) \\ R_i \in \R_2, R_j \in \R_2}}
 \frac{w_i \cdot w_j}{k} + O(W) = O(W)
\end{eqnarray*}


\end{proof}



\begin{figure}
\centering
\begin{minipage}{.3\textwidth}
  \centering
  \includegraphics[width=7cm]{tunnel1.pdf}
\end{minipage}
\begin{minipage}{.3\textwidth}
  \centering
  \includegraphics[width=7cm]{tunnel2.pdf}
\end{minipage}
\begin{minipage}{.3\textwidth}
  \centering
  \includegraphics[width=7cm]{tunnel3.pdf}
\end{minipage}
\caption{$X$ is the first pusher, $Y$ is the second pusher and $Z$ is the third pusher.}
\label{fig:tunnels}
\end{figure}


\begin{lemma}
\label{lemma:disjointcoredecomposition}
Let $\R = \{R_1, \ldots, R_n\}$ be a set of $n$ weighted psuedo-disks,
where $R_i$ has weight $w_i$, and $W = \sum_i w_i$. 
Then there exists
a core decomposition of $\R$, say the set $\tilde{\R} = \{\tilde{R}_1,
\ldots, \tilde{R}_n\}$, such that the disks in $\tilde{\R}$ are pairwise disjoint, and
$$\sum_{i} |v(\tilde{R}_i)| \cdot w_i = O(W \log W)$$
\end{lemma}
\begin{proof}
Each disk $\tilde{R}_i \in \tilde{\R}$ will be composed of pieces
of boundaries of the disks in $\R$. The sequence of the endpoints of these pieces
will be the vertices defining $\tilde{R}_i$ (denote this sequence
by $v(\tilde{R}_i)$).
The information needed to
uniquely determine $\tilde{R}_i$ then is the sequence of these pieces,
or equivalently, the sequence of vertices  defining $\tilde{R}_i$. 
%Set
%the weight of each piece (and vertex) defining $\tilde{R}_i$ to be the weight of $R$,
%and the weight of $\tilde{R}$ to be the sum of the weights of its pieces (equivalently, sum of the weight of its vertices).
%, namely
%$$ weight(\tilde{R}_i) = |v(\tilde{R}_i)| \cdot w_i $$
Then
$$ \sum_{i}
|v(\tilde{R}_i)| \cdot w_i = 
\sum_{(v,i,j)} \sum_{l \text{ s.t. } v \in \tilde{R}_l} w_l
= \sum_{(v,i,j)} \sum_{l \text{ s.t. } v \in R_l} X_{(v,i,j,l)} \cdot w_l $$ 
where the indicator variable $X_{(v,i,j,l)} =1 $ iff $v \in \tilde{R}_l$.
The algorithm to construct $\tilde{\R}$ is the following.

Construct a permutation, say $\pi$, of $\R$ randomly w.r.t. to the weight distribution
of the disks -- pick a random disk, where $R_i$ is picked with probability 
$w_i/W$. Set this disk to be the first disk in the permutation, and recursively
construct the rest of the permutation on the remaining disks. Let $\pi_i$
denote the position of $R_i$ in this permutation. 
Let $\R_0 = \R$. Apply Lemma~\ref{lemma:pusher} (with $R_{\pi^{-1}(1)} \in \R_0$ as the pusher) 
to get a core decomposition, denoted by $\R_1$,
of $\R_0$. Now apply Lemma~\ref{lemma:pusher} on $\R_1$
(with $\tilde{R}_{\pi^{-1}(2)} \in \R_1$ as the pusher) to get the set
$\R_2$. 
Continuing iteratively by applying
Lemma~\ref{lemma:pusher} with the successive core of each $R_{\pi^{-1}(i)}$ in
$\R_i$ as the pusher,
we get the set $\tilde{\R} = \R_n$. See Figure~\ref{fig:tunnels} for an example.

%Let $\mathcal{E}_{(v,i,j)}$ be the event that $\max \{\pi_i, \pi_j\} 
%< \min_{R_m \ni v} \pi_m$, and the random variable
%$X_{(v,i,j)} = 1$ iff $\mathcal{E}_{(v,i,j)}$ occurs.
We have the following crucial fact:
\begin{claim}
If $v(\tilde{R}_l)$ has a vertex corresponding to $(v,i,j)$, 
 then $(v,i,j) \in R_l$ and further
\[ \left\{
  \begin{array}{l l}
    \max \{\pi_i, \pi_j \} < \min_{R_m \ni v} \pi_m & \quad \text{if } l \neq i,j \\
    \pi_j < \pi_i & \quad \text{if } l = i \\
    \pi_i < \pi_j & \quad \text{if } l=j
  \end{array} \right.\]
\end{claim}
\begin{proof}
First consider the case when $l \neq i,j$. 
The proof follows directly from the observation that by the proof of Lemma~\ref{lemma:pusher},
if $v$ is a vertex in the arrangement of $\R$, and at any point a region
containing $v$ in its interior is used as a pusher, then
any  $\tilde{R} \in \tilde{\R}$ cannot have a vertex that corresponds
to $v$.
For the case when $l = i$ (same for when $l=j$), the proof follows from the fact that 
if at any point there are two regions $X$ and $Y$ and $X$ is used as a pusher
before $Y$, then the core of $X$ cannot have a vertex that corresponds to 
a vertex defined by $X$ and $Y$ (see Figure~\ref{fig:twodisks2}).
%vertices to the core of $X$.
%
%Then if some $R_m$ such that
%$(v,i,j) \in R_m$ pushed before $R_i$ or $R_j$, then by the proof of Lemma~\ref{lemma:pusher},
%observe that all vertices inside $R_m$ will not appear as corresponding vertices
%to any other $\tilde{R}$, a contradiction. 
\end{proof}

Using the above Claim and Claim~\ref{claim:cs}, we calculate the expected value of the required bound:

\begin{eqnarray*}
\sum_{i} E \big[ |v(\tilde{R}_i)|  \big] \cdot w_i & = & \sum_{(v,i,j)} \sum_{l \text{ s.t. } v \in R_l} E \big[ X_{(v,i,j,l)}  \big]\cdot w_l \\
& = & \sum_{(v,i,j)} \sum_{l \text{ s.t. } v \in R_l} \Pr \big[ v \in \tilde{R}_l  \big]\cdot w_l \\
& = & \sum_{(v,i,j)} \Bigl( \Pr[ v \in \tilde{R}_i]w_i + \Pr[ v \in \tilde{R}_j]w_j
+ \sum_{\substack{i,j \neq l \\ v \in R_l}}  \Pr[ v \in \tilde{R}_l]w_l \Bigr) \\
& = & \sum_{(v,i,j)} \Bigl( \frac{w_j}{w_i+w_j+d_v}\frac{w_i}{w_i+d_v}w_i  
+ \frac{w_i}{w_i+w_j+d_v}\frac{w_j}{w_j+d_v}w_j \\
& & 
+ \sum_{\substack{i,j \neq l \\ v \in R_l}}  (\frac{w_j}{w_i+w_j+d_v}\frac{w_i}{w_i+d_v}  + \frac{w_i}{w_i+w_j+d_v}\frac{w_j}{w_j+d_v})   w_l  \Bigr) \\
&=& \sum_{(v,i,j)} \Bigl(  
( \frac{w_j}{w_i+w_j+d_v}\frac{w_i}{w_i+d_v} ) \cdot (w_i + \sum_{R_l \ni v} w_l) \\
&& + (\frac{w_i}{w_i+w_j+d_v}\frac{w_j}{w_j+d_v}) \cdot (w_j + \sum_{R_l \ni v} w_l) \Bigr) \\
& = &  2 \sum_{(v,i,j)}  \frac{w_i \cdot w_j}{w_i+w_j+d_v}
 = 2 \sum_k \sum_{\substack{(v,i,j) \\ 2^k \leq d_v < 2^{k+1}}}  \frac{w_i \cdot w_j}{w_i+w_j+d_v} = O(W \log W).
\end{eqnarray*}
where the last inequality follows from Claim~\ref{claim:cs}.
\end{proof}


%\subsection{Weighted pseudo-disk rectangles}

We are now ready to show the existence of a suitable separator. We first give a proof of the existence of the separator for uniformly weighted pseudodisks and then give a different proof for the arbitrary weights case.

\begin{lemma}\label{lem:dayofthejackal}
Given a set of $\mathcal{R}$ of $n$ uniformly weighted $\alpha$-simple pseudodisks (each with weight $1$) and set $P$ of points in the plane, no point lying on the boundary of any of the regions, and any parameter $\delta$, there exists a curve $\C$ such that 
\begin{itemize}
\item $w(\textsc{Opt}(\mathcal{R}, P_{in}(\C))) \leq (\frac{2}{3}+\delta) w(\textsc{Opt}(\mathcal{R}, P))$
\item $w(\textsc{Opt}(\mathcal{R}, P_{ext}(\C))) \leq (\frac{2}{3}+\delta)w(\textsc{Opt}(\mathcal{R}, P))$
\item $w(\textsc{Opt}(\mathcal{R}, P_{in}(\C))) + w(\textsc{Opt}(\mathcal{R}, P_{ext}(\C)))  \leq (1+\delta)w(\textsc{Opt}(\mathcal{R}, P))$
\item the complexity of $\C$ is  $O(\log^5 n/\delta^5)$ 
\end{itemize}
where $w(\mathcal{S})$ denotes the total weight of the regions in $\mathcal{S}$.
\end{lemma}
\begin{proof}
Consider the set $\mathcal{Q} = \textsc{Opt}(\mathcal{R}, P)$. We apply Lemma~\ref{lemma:coredecomposition} to $\mathcal{Q}$ and get
a core decomposition with 
 a core $\tilde{Q}$ for each $Q \in \mathcal{Q}$. Since, the regions in $Q$ cover $P$, their cores also cover $P$.\footnote{Since no point lies on the boundary of any of the regions, there is suitable choice of $\beta$ so that using $\beta$-core decompositions, we do not miss any of the points.} 
By the property of the core decomposition of Lemma~\ref{lemma:coredecomposition},
we have the total number of intersections to be $m = O(\delta^2 n^2 /\log^2 n)$,
and each core has $O(\log^4 n/\delta^4)$ vertices.
Since each of the curves forming the boundary of any core is composed of at most $\alpha$ $x$-monotone curves, the cores are $\alpha_1$-simple for $\alpha_1 = O(\alpha \log^4 n/\delta^4)$.
Applying Theorem~\ref{thm:separator} to these cores with parameter 
$r = \alpha^2 \log^{10} n / \delta^{10}$, we get a curve $\C$, where
\begin{eqnarray*}
\text{Number of cores intersected by }  \C &=& O( \sqrt{m+\alpha_1^2 n^2/r} )
= O(  \sqrt{ \frac{\delta^2 n^2}{\log^2 n} } )  = O( \frac{\delta n}{\log n} ) \\
\text{Complexity of } \C &=& O( \sqrt{r +\frac{mr^2}{\alpha_1^2 n^2}} ) 
= O( \sqrt{\frac{\log^{10}n}{\delta^{10}}} ) = O(\frac{\alpha \log^5 n}{\delta^5})
\end{eqnarray*}

Let $\mathcal{Q}_1$ ($\mathcal{Q}_2$) be the set of regions whose cores are in $interior(\C)$ ($exterior(\C)$).
Let $\mathcal{Q}_3 = \mathcal{Q} \setminus \{\mathcal{Q}_1 \cup \mathcal{Q}_2\}$. 
Observe that the cores of the regions in $\mathcal{Q}_{1} \cup \mathcal{Q}_{3}$ cover all the points in $P_{in}$ and therefore the regions in $\mathcal{Q}_{1} \cup \mathcal{Q}_{3}$ themselves cover the points in $P_{in}$. Similarly the regions in $Q_{2} \cup \mathcal{Q}_{3} $ cover the points in $P_{ext}$.
Theorem~\ref{thm:weightedseparator} guarantees that $w(\mathcal{Q}_{1})$ and $w(\mathcal{Q}_{2})$ are at most $\frac{2}{3}w(\mathcal{Q})$ and $w(\mathcal{Q}_{3}) \leq \delta w(\mathcal{Q})$. Therefore, 
$$w(\textsc{Opt}(\mathcal{R}, P_{in})) \leq w(\mathcal{Q}_{1} \cup \mathcal{Q}_{3}) = w(\mathcal{Q}_{1}) + w(\mathcal{Q}_{3}) \leq (\frac{2}{3}+\delta)w(\mathcal{Q})$$
This proves the first item in the statement of the theorem. The second item is proved analogously. For the third item, we combine the inequalities $w(\textsc{Opt}(\mathcal{R}, P_{in})) \leq w(\mathcal{Q}_{1}) + w(\mathcal{Q}_{3})$ and $w(\textsc{Opt}(\mathcal{R},P_{ext})) \leq w(\mathcal{Q}_{2}) + w(\mathcal{Q}_{3})$. We get 
$$w(\textsc{Opt}(\mathcal{R}, P_{in})) + w(\textsc{Opt}(\mathcal{R}, P_{ext})) \leq w(\mathcal{Q}_{1}) + w(\mathcal{Q}_{2}) + 2w(\mathcal{Q}_{3}) \leq w(\mathcal{Q}) + w(\mathcal{Q}_{3}) \leq (1+\delta)w(\mathcal{Q})$$ 
That proves the third item. 
Lemma~\ref{lemma:coredecomposition} also gives a set $\Gamma(\tilde{Q})$ for each $Q\in \mathcal{Q}$. Let $Y = \cup_{Q\in \mathcal{Q}} \Gamma(\tilde{Q})$. The separator $\C$ given by Theorem~\ref{thm:separator} can be described by a sequence of $O(\alpha\log^5 n/\delta^5)$ curves in $Y$ and $O(\alpha\log^5 n/\delta^5)$ additional bits. Since, by Lemma~\ref{lemma:coredecomposition} each curve in $Y$ can be described by a sequence of at most three curves in $\Gamma(\mathcal{R})$ and a constant number of bits, $\C$ can also be described by a sequence of  $O(\alpha\log^5 n/\delta^5)$ curves in $\Gamma(\mathcal{R})$ and $O(\alpha\log^5 n/\delta^5)$ additional bits of information.
\end{proof}

Following what we did in Section~\ref{sec:mis}, we set $\delta =c \epsilon/\log{\frac{n}{\epsilon}}$ with a suitable constant $c$ such that $\delta < 1/3$. 
This ensures that the size of the optimal solution goes down by a constant factor in both the subproblems created by the separator given by Lemma~\ref{lem:dayofthejackal}.
This time there are $(\alpha n)^{O(\alpha\log^5{n}/\delta^5)}$ candidate separators for each subproblem. Thus, by an algorithm similar to that described in Section~\ref{sec:mis}, we conclude  Theorem~\ref{thm:setcover} for the case of uniform weights.

Next we prove the existence of a suitable separator for the case of arbitrary weights. Recall that one can assume without loss of generality that the minimum weight is $1$. 

\begin{lemma}\label{lem:rajnikant}
Let $\mathcal{R}$ be a set of $n$ weighted $\alpha$-simple pseudodisks with each pseudodisk having a minimum weight $1$ and no pseudodisk having a weight more than a third of the total weight. Let $P$ be a set of points in the plane, with no point lying on the boundary of any of the pseudodisks. Then for $\delta$, there exists a curve $\C$ such that 
\begin{itemize}
\item $w(\textsc{Opt}(\mathcal{R}, P_{in}(\C))) \leq (\frac{2}{3}+3\delta) w(\textsc{Opt}(\mathcal{R}, P))$
\item $w(\textsc{Opt}(\mathcal{R}, P_{ext}(\C))) \leq (\frac{2}{3}+3\delta)w(\textsc{Opt}(\mathcal{R}, P))$
\item $w(\textsc{Opt}(\mathcal{R}, P_{in}(\C))) + w(\textsc{Opt}(\mathcal{R}, P_{ext}(\C)))  \leq (1+2\delta)w(\textsc{Opt}(\mathcal{R}, P))$
\item The complexity of $\C$ is $O(\frac{\alpha}{\delta^2} \log w(\textsc{Opt}(\R,P))$.
\end{itemize}
where $w(\mathcal{S})$ denotes the total weight of the regions in $\mathcal{S}$.
\end{lemma}
\begin{proof}
The proof is very similar to the proof of Lemma~\ref{lem:dayofthejackal}.
This time, we use
Lemma~\ref{lemma:disjointcoredecomposition} to obtain a core $\tilde{Q}$ for each $Q 
\in \Q = \textsc{Opt}(\R,P)$ and we assign to $\tilde{Q}$ the same weight as $Q$. 
We denote the number of vertices in $\tilde{Q}$ by $v(\tilde{Q})$. 
By Lemma~\ref{lemma:disjointcoredecomposition}, $\sum_{Q \in \Q} v(\tilde{Q}) w(Q) = O(w(\Q)
 \log{w(\Q)}))$. It follows that if we set $\tau = C\cdot\frac{1}{\delta}\log{w(\Q)}$ for some large enough constant $C$,
 then $\sum_{Q \in \Q: v(\tilde{Q}) >\tau } w(Q) < \delta w(\Q)$.
  Let $\Q_1 = \{ Q \in \Q: v(\tilde{Q}) \leq \tau \}$ and let $\tilde{\Q}_1 = \{ \tilde{Q} : Q \in \Q_1 \}$.
  
The regions in $\tilde{\Q}_1$ are $\alpha\tau$-simple since they have at most $\tau$ sides and 
each of the sides is a portion of the boundary of a single $\alpha$-simple region in $\R$.
These regions have a total weight of $w(\Q_1)$. Thus applying Theorem~\ref{thm:weightedseparator}, we get separator $\C$ so that the total weight of the regions of $\Q$ whose cores lie completely
 inside or outside $\C$ is at most $\frac{2}{3}w(\Q_1)$. Since the total weight of the regions in
  $\Q \setminus \Q_1$ is at most $\delta w(\Q)$, the total weight of all the cores that lie
   completely inside (or completely outside) $\C$ is at most $(\frac{2}{3}+\delta)w(\Q)$. Also, the
    total weight of the cores in $\Q_1$ that intersect $\C$ is at most $\delta w(\Q_1)$. Thus the
     total weight of all the cores in $\Q$ that intersect $\C$ is at most $2\delta w(\Q)$. The complexity of $\C$ is $O(\alpha\tau/\delta) = O(\frac{\alpha}{\delta^2} \log{w(\Q)} )$.

The rest of the proof is exactly the same as in the proof of Lemma~\ref{lem:dayofthejackal}.
\end{proof}

To finish the proof of Theorem~\ref{thm:setcover}, we first use Claim~\ref{claim:tofame} to reduce the given instance of the set cover problem to an instance $(\R,P)$ where the minimum weight of the regions is $1$ and the weight of the optimal solution $w(\textsc{Opt}(\R,P))$ is $O(n/\epsilon)$. The input instance can be easily perturbed so that no point lies on the boundary of any of the regions.
 As in Section~\ref{sec:mis}, we set $\delta =c \epsilon/\log{(n/\epsilon)}$ with a suitable constant $c$ and $\delta < 1/9$ 
to ensures that the size of the optimal solution goes down by a constant factor in both the subproblems created by the separator curve given by Lemma~\ref{lem:rajnikant}.
 The complexity of the separator is $O(\frac{\alpha}{\delta^2}\log{\frac{n}{\epsilon}})$.
Thus there are $(\alpha n)^{O(\frac{\alpha}{\delta^2}\log{\frac{n}{\epsilon}})} = (\alpha n)^{O(\frac{\alpha}{\epsilon^2}\log^3{\frac{n}{\epsilon}})}$ candidate separators for each subproblem. By an algorithm similar to that in Section~\ref{sec:mis}, we conclude  Theorem~\ref{thm:setcover}.\\

{\bf Remark:} Theorem~\ref{thm:setcover} can be extended to work for more general regions called {\em non-piercing regions} or {$r$-admissible regions}. For this only Lemma~\ref{lemma:pusher} needs to be extended to work for these regions. Everything else works as it is. In this case, a region $R$ may intersect the boundary of pusher $X$ in more than one interval. To ensure that after pushing the new regions are still non-piercing, different gaps are required in different intervals for the same region $R$. This makes it technically more complicated but no new idea is involved.

\subsection{Lower bounds}
\label{observation:lowerbound}
In this section we give examples of regions of low (but superlinear) union complexity that do not admit a PTAS.

\begin{observation}
The problem of approximating minimum-size set-cover is:
\begin{enumerate}
\item APX-hard for a set $\R$ of $n$ $4$-sided polygons in the plane
of union complexity $n \alpha (n)$.
\item inapproximable within $o(\log s)$ factor for a set $\R$ of $n$ $4s$-sided polygons in the plane
of union complexity $n 2^{\alpha(n)^{O(s)}}$, for any integer $s>3$.
\end{enumerate}
\end{observation}
\begin{proof}
Chan-Grant~\cite{CG2014} showed that computing minimum size set-covers
for objects defined by shadows of line-segments in the plane is APX-hard. 
By Davenport-Schinzel sequences, the union complexity of $n$ line-segments in the plane 
is $O(n \alpha(n))$. These shadows can be `closed off' without any further
intersections to derive the $4$-sided polygons, proving 1.

Trevisan~\cite{Trevisan01} showed that computing minimum size set-covers
for general set systems $(V, \{S_1, \ldots, S_m\})$ where each $S_i$ has size $O(s)$
is inapproximable with factor $o(\log s)$ unless $P = NP$. 
These sets can be easily implemented using regions whose boundaries cross at most $O(s)$ times. To see this place a point corresponding to each vertex on the $x$-axis. Then for each set $S_i$ construct $x$-monotone curve $\gamma_i$ with $2s+1$ horizontal segments and $2s$ nearly vertical segments so that the points corresponding to the vertices in $S_i$ lie above $\gamma_i$ and all other points lies below $\gamma_i$. 
These curves can easily be drawn in such a way that any two of them intersect at most $O(s)$ times. Thus by bounds known on Davenport-Shinzel sequences, the lower envelope of the curves has complexity $O(n 2^{\alpha(n)^{O(s)}})$.
 Thus if we consider the regions $R_i$ defined by the set of points above $\gamma_i$ we get a set of regions with small union complexity. These regions can be
 made bounded without increasing the union complexity.
\end{proof}


